Pay Attention to Hidden States for Video Deblurring: Ping-Pong Recurrent Neural Networks and Selective Non-Local Attention

Video deblurring models exploit information in the neighboring frames to remove blur caused by the motion of the camera and the objects. Recurrent Neural Networks~(RNNs) are often adopted to model the temporal dependency between frames via hidden states. When motion blur is strong, however, hidden states are hard to deliver proper information due to the displacement between different frames. While there have been attempts to update the hidden states, it is difficult to handle misaligned features beyond the receptive field of simple modules. Thus, we propose 2 modules to supplement the RNN architecture for video deblurring. First, we design Ping-Pong RNN~(PPRNN) that acts on updating the hidden states by referring to the features from the current and the previous time steps alternately. PPRNN gathers relevant information from the both features in an iterative and balanced manner by utilizing its recurrent architecture. Second, we use a Selective Non-Local Attention~(SNLA) module to additionally refine the hidden state by aligning it with the positional information from the input frame feature. The attention score is scaled by the relevance to the input feature to focus on the necessary information. By paying attention to hidden states with both modules, which have strong synergy, our PAHS framework improves the representation powers of RNN structures and achieves state-of-the-art deblurring performance on standard benchmarks and real-world videos.

==> sections/figs/dvd_split.tex <==
\begin{figure*}[t]
    % \captionsetup[sub]{font=footnotesize}
    \centering
    \renewcommand{\wp}{0.0955\linewidth}
    \includegraphics[width=\wp]{figs/dvd2/blur_1.png}
    \includegraphics[width=\wp]{figs/dvd2/blur_2.png}
    \hfill
    \includegraphics[width=\wp]{figs/dvd2/tsp_1.png}
    \includegraphics[width=\wp]{figs/dvd2/tsp_2.png}
    \hfill
    \includegraphics[width=\wp]{figs/dvd2/arvo_1.png}
    \includegraphics[width=\wp]{figs/dvd2/arvo_2.png}
    \hfill
    \includegraphics[width=\wp]{figs/dvd2/ours_1.png}
    \includegraphics[width=\wp]{figs/dvd2/ours_2.png}
    \hfill
    \includegraphics[width=\wp]{figs/dvd2/gt_1.png}
    \includegraphics[width=\wp]{figs/dvd2/gt_2.png}
    \\
    \renewcommand{\wp}{0.195\linewidth}
    \subfloat[Input]{\includegraphics[width=\wp]{figs/dvd2/blur_full.png}}
    \hfill
    \subfloat[TSP~\cite{Pan_2020_CVPR}]{\includegraphics[width=\wp]{figs/dvd2/tsp_full.png}}
    \hfill
    \subfloat[ARVo~\cite{li2021arvo}]{\includegraphics[width=\wp]{figs/dvd2/arvo_full.png}}
    \hfill
    \subfloat[\textbf{LR-RNN(Ours)}]{\includegraphics[width=\wp]{figs/dvd2/ours_full.png}}
    \hfill
    \subfloat[Ground Truth]{\includegraphics[width=\wp]{figs/dvd2/gt_full.png}}
    \\
    \vspace{-5mm}
    \figcspace
    \caption{Qualitative comparison on the DVD~\cite{Su_2017_CVPR} dataset.
    }
    % \caption{Comparison of baselines and RIRN-applied method results}
    \label{fig:dvd_split}
    \vspace{3mm}
    \figspace
\end{figure*}

==> sections/figs/graph-binum.tex <==
\begin{figure}[t]
    \renewcommand{\wp}{0.9\linewidth}
    \centering
    \subfloat[Effect of PPRNN]{\includegraphics[width=\wp]{figs/graph/binum.pdf}}
    \figcspace
    \vspace{-5mm}
    \caption{
    }
    % \caption{Comparison of baselines and RIRN-applied method results}
    \vspace{3mm}
    \label{fig:binum-graph}
    \figspace
\end{figure}

==> sections/figs/hiddens.tex <==
\begin{figure}[t]
    \renewcommand{\wp}{0.3\linewidth}
    
    \centering
    % \captionsetup[sub]{font=footnotesize}
    \subfloat[$L_{t-1}$]{\includegraphics[width=\wp]{figs/hiddenstates/deblur1.png}}
    \hfill
    \subfloat[$I_{t}$]{\includegraphics[width=\wp]{figs/hiddenstates/blur2.png}}
    \hfill
    \subfloat[$L_{t}$]{\includegraphics[width=\wp]{figs/hiddenstates/deblur2.png}}
    \\
    \subfloat[$R_{t-1}$\label{fig:d}]{\includegraphics[width=\wp]{figs/hiddenstates/hidden_ori.png}}
    \hfill
    \subfloat[$H_{t}$\label{fig:e}]{\includegraphics[width=\wp]{figs/hiddenstates/hidden_before.png}}
    \hfill
    \subfloat[$NLH_{t}$\label{fig:f}]{\includegraphics[width=\wp]{figs/hiddenstates/hidden_after.png}}
    \figcspace
    \vspace{-5mm}
    \caption{Visualization of the hidden states. When neighboring deblurred frame is (a) and target frame is (b), (d) shows hidden state extracted without referencing (b). Without PPRNN and SNLA, (d) itself is delivered to the target frame. However hidden state extracted by using PPRNN is shown as (e) and with SNLA (f) is delivered to the target feature. (c) is the final restored result from (b) in our model.
    }
    % \caption{Comparison of baselines and RIRN-applied method results}
    \vspace{3mm}
    \label{fig:hiddens}
    \figspace
\end{figure}

==> sections/figs/model.tex <==
\begin{figure*}[t]
    \centering
    \renewcommand{\wp}{0.99\linewidth}
    % \captionsetup[sub]{font=footnotesize}
    \includegraphics[width=\wp]{figs/model2.pdf}
    \figcspace
    \vspace{-5mm}
    \caption{
        Overview of the proposed video deblurring method. Our method first extract the feature from the target frame. With PPRNN, the model extract the relevant hidden states referencing the target feature. Then it computes the non local attention selectively between the hidden state and the target feature. Finally, we obtain deblurred frame from a reconstruction network. 
    }
    % \caption{Comparison of baselines and RIRN-applied method results}
    \label{fig:model}
    \vspace{3mm}
    \figspace
\end{figure*}

==> sections/figs/pprnn.tex <==
\begin{figure}[t]
    \centering
    \renewcommand{\wp}{0.99\linewidth}
    % \captionsetup[sub]{font=footnotesize}
    \includegraphics[width=\wp]{figs/PPRNN2.pdf}
    \vspace{-5mm}
    \figcspace
    \caption{
         Illustration of the PPRNN module. PPRNN extract the hidden states referencing the target frame. 
         Exchanging process between the hidden state and the target feature is denoted as $VN$. We set $VN=1$ for the figure.
    }
    % \caption{Comparison of baselines and RIRN-applied method results}
    \label{fig:pprnn}
    \figspace
\end{figure}

==> sections/figs/snla.tex <==
\begin{figure}[t]
    \centering
    \renewcommand{\wp}{0.99\linewidth}
    % \captionsetup[subfloat]{font=footnotesize}
    \includegraphics[width=\wp]{figs/SNLA2.pdf}
    \vspace{-5mm}
    \figcspace
    \caption{
        Illustration of the SNLA module. SNLA selectively aggregate the features for target feature using non-local attention and an additional sigmoid layer. Also for memory saving, it is consist of encoder-decoder structure.
    }
    \label{fig:snla}
    \vspace{3mm}
    \figspace
\end{figure}

==> sections/tables/overallDVD.tex <==
\begin{table}[t]
    \footnotesize
        \resizebox{1.0\linewidth}{!}{
        \begin{tabular}{c|cccccccc}
            \toprule
            Methods & EDVR~\cite{Wang_2019_CVPR_Workshops} & OVD~\cite{Kim_2017_ICCV} & IFI-RNN~\cite{Nah_2019_CVPR}& STFAN~\cite{Zhou_2019_ICCV} & 
            ESTRNN~\cite{zhong2020efficient} & 
            TSP~\cite{Pan_2020_CVPR}  & ARVo~\cite{li2021arvo} & \textbf{PAHS}\\
            \midrule
            PSNR & 28.51 & 29.15 &  30.53 & 31.15 & 31.92 & 32.13  & \uline{32.65} & \textbf{33.28}\\
            SSIM & 0.8637 & 0.8728 &  0.9069 & 0.9049 & 0.9298 & 0.9268 & \uline{0.9352} & \textbf{0.9565}\\
            \midrule
            Model Size(MB) & 20.6 & 1.4  & 3.6 & 5.4 & 2.5 & 16.1 & 20.6 &  21.0 \\
            Speed (fps) & 2.70 & 7.69 & 20.15 & 6.66 & 6.21 & 0.22 & 0.15 &  1.43\\
            \bottomrule
        \end{tabular}
        }
    \tabcspace
    \caption{
    \textbf{Quantitative comparison with state-of-the-art methods on DVD~\cite{Su_2017_CVPR} dataset.}
    A single NVIDIA GTX 1080 Ti GPU is used for evaluating speed.
    }
    \label{tab:DVD}
    \vspace{-9mm}
    % \tabspace
\end{table}



==> sections/tables/overallDVD2.tex <==
\begin{table*}[t]
% \captionsetup[subfloat]{font=footnotesize}
\caption{Deblurring accuracy comparison on the DVD~\cite{Su_2017_CVPR} dataset. We evaluate the model with PSNR and SSIM metrics considering all the restored video frames.
Although ARVo~\cite{li2021arvo} shows slight better performance in PSNR, it requires \textbf{4 times} more parameters and \textbf{27.8 times} more time to deblur the video than our PAHS-RNN.
}
\label{tab:DVD}
\scriptsize
\resizebox{1.0\linewidth}{!}{\begin{tabular}{c|ccccccccc}
        \toprule
        Methods & EDVR~\cite{Wang_2019_CVPR_Workshops} & STRCNN~\cite{Kim_2017_ICCV} & DBN~\cite{Su_2017_CVPR} & IFIC1 ~\cite{Nah_2019_CVPR}& STFAN~\cite{Zhou_2019_ICCV} & TSP~\cite{Pan_2020_CVPR}  & ARVo~\cite{li2021arvo} & \textbf{PAHS-RNN} & \textbf{PAHS-RNN(L)}\\
        \midrule
        PSNR & 28.51 & 29.15 &  30.01 & 30.53 & 31.15 & 32.13  & 32.80 & 32.65 & \textbf{33.28}\\
        SSIM & 0.8637 & 0.8728 &  0.8877 & 0.9069 & 0.9049 & 0.9268  & 0.9352 & 0.9459 & \textbf{0.9565}\\
        \bottomrule
    \end{tabular}}
    \tabspace
    \vspace{3mm}
\end{table*}


==> sections/tables/pprnn.tex <==
\begin{table}[t]
    % \captionsetup[subfloat]{font=footnotesize}
    \label{tab:PPRNN}
    \tabcspace
    \centering
    \vspace{-5mm}
    \begin{tabular}{c|cc|c|c}
        \toprule
        num of cell & PSNR & SSIM & time(second)& params(MB)\\
        \midrule
        0 & 31.83 & 0.9398 & 0.22 & 4.2\\
        \textbf{1} & 32.77 & 0.9492 & 0.24 & 5.3 \\
        1 & 32.82 & 0.9522 & 0.27 & 6.3\\
        2 & 32.79 & 0.9524 & 0.31 & 7.3\\
        \bottomrule
    \end{tabular}
    \caption{Effects of using PPRNN.}
    \tabspace
    \vspace{3mm}
\end{table}

==> sections/tables/snla.tex <==
% \begin{table}[t]
%     % \newcommand{\cmark}{\ding{51}}%
%     \newcommand{\cmark}{\textcolor{MyGreen}{\ding{51}}}
%     \newcommand{\xmark}{\ding{55}}%
%     %We desinged SNLA with additional filtering module with encoder-decoder mechanism as shown in Figure~\ref{fig:snla}. We do ablation study comparing our full model with several models without using SNLA module and without using filtering module in the SNLA.}
%     \centering
%         \begin{tabular}{c|cc|cc}
%             \toprule
%             Method & Attention & Filtering module & PSNR & SSIM \\
%             \midrule
%             Baseline & \xmark & \xmark & 31.02 & 0.9091 \\
%             NLA & \cmark & \xmark & 32.49 & 0.9371 \\
%             \textbf{SNLA} & \cmark & \cmark & \textbf{32.66} & \textbf{0.9484}\\
%             \bottomrule
%         \end{tabular}
%     \caption{\textbf{Effect of SNLA and its components.} Both the attention and filtering modules make substantial contribution to the performance improvement.} 
%     \label{tab:snla}
%     \tabspace
% \end{table}
